Unpacking .zip: A First Look at Domain and File Name Confusion

The namespace for filenames and DNS names has overlapped since the introduction of DNS in 1985: \texttt{.com} was the original binary format used for DOS and CP/M systems. Recently the introduction of gTLDs such as \texttt{.zip} and \texttt{.mov}, coupled with the growing prevalence of web resources, has ignited new concerns about potential issues related to DNS and filename confusion. Thus far, the discourse on DNS/filename confusion has been piecemeal and hypothetical, making it unclear what, if any, security concerns credibly exist. To address this gap, we provide the first enumeration of how DNS/filename confusion can be abused. We then perform the first empirical case studies of DNS/filename confusion in the wild, which highlights suspected confusion across a wide range of software. Finally, based on our preliminary findings, we provide suggestions and guidance for future research on this topic.

==> sections/03-methodology.tex <==
\section{Methodology}




==> sections/05-filesquatting_domains.tex <==
\section{Filesquatting Domains}

% Using a passive DNS dataset of a North American ISP from 2024-01 to 2024-10 \todo{double check \& get more specific?}, we examined the most frequently queried domains with file extension TLDs. 

% To do this, we first filtered out any domains that were already registered as well as domains that did not have common file extension TLDs. Next, we sorted the domains based on the number of queries that they received. Lastly, prioritizing domains with the most queries, we manually chose domains that most resembled file names.

% From our final list of domains that were not yet registered, resembled file names, and were receiving many (greater than 1,000 lookups), we registered four domains: \texttt{gitlab.zip}, \texttt{crowdstrike-hotfix.zip}, \texttt{downloaddataen.zip}, and \texttt{wallboard-generic-oreo-ota-2022\_02\_17-10\_54\_31-signed.zip}. In addition to domains sourced from the passive DNS data, we decided to register two additional domains opportunistically that resembled file names: \texttt{meharmtadata.zip} and \texttt{manifest.zip}. Table 2 lists these domains with the number of queries that were observed in the passive DNS data. Lastly, the domains \texttt{manifest.observer} and \texttt{metadata.rodeo} were registered to serve as a baseline for regular internet scanner traffic.

% \begin{table}
%     \centering
%     \begin{tabular}{l c}
%          \textbf{Domain} & \textbf{\# Lookups} \\
%          \hline\hline
%          gitlab.zip & 331,810 \\
%          wallboard-generic-oreo-[...].zip & 59,773 \\
%          crowdstrike-hotfix.zip & 7,709 \\
%          downloaddataen.zip & 3,128 \\
%          metadata.zip & N/A \\
%          manifest.zip & N/A \\
%     \end{tabular}
%     \caption{Number of lookups observed in passive DNS data}
%     \label{tab:my_label}
% \end{table}


==> sections/08-ethics.tex <==
\section*{Ethics}

This study involved the controlled registration of a small number of domains under newly introduced TLDs for the purpose of observing automatic auto-linking and link preview behavior. All domains were operated as non-interactive honeypots that served static, benign responses and collected only minimal, non-identifiable metadata from incoming HTTP requests. NO content resembling legitimate services or brands was hosted, and no user interaction or credential submission was solicited or possible. IP addresses were analyzed only at the network level (e.g., ASN, country), and no attempt was made to correlate them with specific individuals.

\todo{Comment on crowdstrike}


